GAP-RL: Grasps As Points for RL Towards Dynamic Object Grasping

Dynamic grasping of moving objects in complex, continuous motion scenarios remains challenging. Reinforcement Learning (RL) has been applied in various robotic manipulation tasks, benefiting from its closed-loop property. However, existing RL-based methods do not fully explore the potential for enhancing visual representations. In this letter, we propose a novel framework called Grasps As Points for RL (GAP-RL) to effectively and reliably grasp moving objects. By implementing a fast region-based grasp detector, we build a Grasp Encoder by transforming 6D grasp poses into Gaussian points and extracting grasp features as a higher-level abstraction than the original object point features. Additionally, we develop a Graspable Region Explorer for real-world deployment, which searches for consistent graspable regions, enabling smoother grasp generation and stable policy execution. To assess the performance fairly, we construct a simulated dynamic grasping benchmark involving objects with various complex motions. Experiment results demonstrate that our method effectively generalizes to novel objects and unseen dynamic motions compared to other baselines. Real-world experiments further validate the framework's sim-to-real transferability.

==> tables/ablations.tex <==
% Ours & $\textbf{0.580}\pm\textbf{0.022}$ & $\textbf{0.531}\pm\textbf{0.027}$ & 
% $\textbf{0.510}\pm\textbf{0.021}$ & $\textbf{0.457}\pm\textbf{0.025}$ & 
% $\textbf{0.487}\pm\textbf{0.040}$ & $\textbf{0.430}\pm\textbf{0.028}$\\
% Ours (fix-shape) & $0.347\pm0.102$ & $0.320\pm0.087$ & 
% $0.270\pm0.065$ & $0.243\pm0.066$ & 
% $0.297\pm0.049$ & $0.260\pm0.048$ \\
% Ours (GPG $\rightarrow$ PN) & $0.452\pm0.024$ & $0.413\pm0.020$ & 
% $0.438\pm0.057$ & $0.403\pm0.041$ & 
% $0.357\pm0.064$ & $0.310\pm0.045$ \\

% \begin{table}[t]
% \centering
% \caption{Ablations on Grasp Pose Descriptor.}
% \label{tab:ablation}
% \renewcommand\arraystretch{1.3}
% \setlength{\tabcolsep}{2mm}
% \small
% \begin{tabularx}{1.0\linewidth}{cccc}
% \hline
% \textbf{Methods}  & $L=16$ & $L=32$ & $L=64$ \\ \hline
% GP $\xrightarrow$ KP & $0.348\pm0.072$ & $0.377\pm0.066$ & $0.408\pm0.088$ \\
% GGN $\xrightarrow$ PN & $0.423\pm0.051$ & $0.467\pm0.065$ & $0.459\pm0.064$ \\ 
% Ours & $\textbf{0.481}\pm\textbf{0.050}$ & $\textbf{0.502}\pm\textbf{0.054}$ & $\textbf{0.489}\pm\textbf{0.049}$\\ \hline
% \end{tabularx}
% \vspace{-1mm}
% % \vspace{-1em}
% \end{table}

==> tables/dynamic_settings.tex <==
\begin{table}[t]
\caption{Parameters for motion types.}
\label{Tab.SimSetup}
\centering
\tabcolsep=0.15cm
\renewcommand\arraystretch{1.1}
\begin{threeparttable}
\begin{tabular}{l|ccccc}
\Xhline{1.5pt}
Type & $l(m)$ & $r(m)$ & $\theta(^\circ)$ & $v(m/s)$ \\
\hline
Rotation & $0.6$ & $[0.18, 0.22]$ & - & $0$  \\
Line & $[0.55, 0.65]$ & - & $[-30, 30]$  & $[-0.06, 0.06]$  \\
Circle & $[0.55, 0.65]$ & $[0.1, 0.2]$  & -  & $[-0.06, 0.06]$  \\
Random & $0.6$ & $[0.18, 0.22]$  & - & $[-0.06, 0.06]$  \\
\Xhline{1.5pt}
\end{tabular}
% $^\ast$ $\omega \in [-10^\circ, 10^\circ]$ is the rotation angular velocity around the \textit{z}-axis. $d$ means the direction of $v$.
\vspace{-0.5cm}
\end{threeparttable}
\end{table}
